Reinforcement Learning and Tree Search Methods for the Unit Commitment Problem

The unit commitment (UC) problem, which determines operating schedules of generation units to meet demand, is a fundamental task in power systems operation. Existing UC methods using mixed-integer programming are not well-suited to highly stochastic systems. Approaches which more rigorously account for uncertainty could yield large reductions in operating costs by reducing spinning reserve requirements; operating power stations at higher efficiencies; and integrating greater volumes of variable renewables. A promising approach to solving the UC problem is reinforcement learning (RL), a methodology for optimal decision-making which has been used to conquer long-standing grand challenges in artificial intelligence. This thesis explores the application of RL to the UC problem and addresses challenges including robustness under uncertainty; generalisability across multiple problem instances; and scaling to larger power systems than previously studied. To tackle these issues, we develop guided tree search, a novel methodology combining model-free RL and model-based planning. The UC problem is formalised as a Markov decision process and we develop an open-source environment based on real data from Great Britain's power system to train RL agents. In problems of up to 100 generators, guided tree search is shown to be competitive with deterministic UC methods, reducing operating costs by up to 1.4\%. An advantage of RL is that the framework can be easily extended to incorporate considerations important to power systems operators such as robustness to generator failure, wind curtailment or carbon prices. When generator outages are considered, guided tree search saves over 2\% in operating costs as compared with methods using conventional $N-x$ reserve criteria.

==> 02-literature/duc_setup.tex <==
\begin{scriptsize}
\renewcommand*{\arraystretch}{1.5}
\begin{longtable}{lrp{1in}p{1.5in}rr}
\toprule
\textbf{Method} &\textbf{Year} &\textbf{Type} &\textbf{Test System(s) \newline (max. units)} &\textbf{Reference} \\\midrule
DP &1966 &Math opt. &Dpt. Water \& Power (14) \cite{lowery1966generating} &\cite{lowery1966generating} \\
PL &1971 &Heuristic &CONVEX (100) \cite{johnson1971large} &\cite{johnson1971large} \\
DP &1976 &Math opt. &Pang (17) \cite{pang1976optimal} &\cite{pang1976optimal} \\
LR/MILP &1977 &Math opt. &Muckstadt (15) \cite{muckstadt1977application} &\cite{muckstadt1977application} \\
PL &1980 &Heuristic &Texas \cite{shoults1980practical} &\cite{shoults1980practical} \\
LR &1983 &Math opt. &EDF (172) \cite{merlin1983new} &\cite{merlin1983new} \\
DP &1987 &Math opt. &SDG\&E (33) \cite{snyder1987dynamic} &\cite{snyder1987dynamic} \\
LR &1987 &Math opt. &Cohen (13) \cite{cohen1987method} &\cite{cohen1987method} \\
LR &1988 &Math opt. &Bard \cite{bard1988short} (10) &\cite{bard1988short} \\
LR &1988 &Math opt. &Zhuang \cite{zhuang1988towards} (100) &\cite{zhuang1988towards} \\
PL &1988 &Heuristic &EPRI (174) \cite{zaininger1977synthetic} &\cite{lee1988short} \\
LR &1989 &Math opt. &Virmani (20) \cite{virmani1989implementation} &\cite{virmani1989implementation} \\
SA &1990 &Metaheursitic &Turgeon \cite{turgeon1978optimal} (10); Zhuang \cite{zhuang1988towards} (100) &\cite{zhuang1990unit} \\
PL &1990 &Heuristic &Sheble (15) \cite{sheble1990solution} &\cite{sheble1990solution} \\
DP &1991 &Math opt. &Ouyang (26) \cite{ouyang1991intelligent} &\cite{ouyang1991intelligent} \\
GA &1996 &Metaheursitic &Kazarlis \cite{kazarlis1996genetic} (100) &\cite{kazarlis1996genetic} \\
SA &1998 &Metaheursitic &Bard \cite{bard1988short} (10); Turgeon \cite{turgeon1978optimal} (10); Tong \cite{tong1991heuristic} (26) &\cite{mantawy1998simulated} \\
LR &1999 &Math opt. &Bard \cite{bard1988short} (11); Shaw \cite{shaw1995direct} (26) &\cite{hobbs1999analysis} \\
LR &2000 &Math opt. &Kazarlis \cite{kazarlis1996genetic} (100) &\cite{cheng2000unit} \\
GA &2000 &Metaheursitic &Kazarlis \cite{kazarlis1996genetic} (100) &\cite{cheng2000unit} \\
LR/GA &2000 &Math opt./metaheuristic &Kazarlis \cite{kazarlis1996genetic} (100) &\cite{cheng2000unit} \\
GA &2002 &Metaheursitic &Kazarlis \cite{kazarlis1996genetic} (10) &\cite{swarup2002unit} \\
PL &2003 &Heuristic &Kazarlis \cite{kazarlis1996genetic} (100) &\cite{senjyu2003fast} \\
LR &2004 &Math opt. &Kazarlis \cite{kazarlis1996genetic} (100) &\cite{ongsakul2004unit} \\
LR &2005 &Math opt. &IEEE 118 (66) &\cite{li2005price} \\
MILP &2005 &Math opt. &IEEE 118 (66) &\cite{li2005price} \\
LR &2005 &Math opt. &IEEE 118 (54) &\cite{fu2005security} \\
PSO &2006 &Metaheursitic &Kazarlis \cite{kazarlis1996genetic} (100) &\cite{zhao2006improved} \\
MILP &2006 &Math opt. &Kazarlis \cite{kazarlis1996genetic} (100) &\cite{carrion2006computationally} \\
PSO &2006 &Metaheursitic &Kazarlis \cite{kazarlis1996genetic} (10) &\cite{ting2006novel} \\
SA &2006 &Metaheursitic &Kazarlis \cite{kazarlis1996genetic} (100) &\cite{simopoulos2006unit} \\
PSO &2010 &Metaheursitic &Kazarlis \cite{kazarlis1996genetic} (100) &\cite{jeong2010new} \\
MILP &2011 &Math opt. &Kazarlis \cite{kazarlis1996genetic} (187) &\cite{ostrowski2011tight} \\
MILP &2013 &Math opt. &Kazarlis \cite{kazarlis1996genetic} (187) &\cite{morales2013tight} \\
MILP &2013 &Math opt. &IEEE 118 (54) &\cite{amjady2013hydrothermal} \\
PL &2015 &Heuristic &Kazarlis \cite{kazarlis1996genetic} (1000) &\cite{quan2015improved} \\
MILP &2016 &Math opt. &MISO (1400) &\cite{chen2016improving} \\
PL &2017 &Heuristic &Kazarlis \cite{kazarlis1996genetic} (100) &\cite{elsayed2017new} \\
MILP &2017 &Math opt. &Kazarlis \cite{kazarlis1996genetic} (1870); FERC (939) \cite{krall2012rto} &\cite{atakan2017state} \\
MILP &2019 &Math opt. &MISO (1400) &\cite{xavier2019transmission} \\
MILP &2020 &Math opt. &RTS-GMLC (73); CAISO (410); FERC (939) \cite{krall2012rto} &\cite{knueven2020mixed} \\
\bottomrule
\caption{Summary of selected deterministic UC studies. The methods reviewed in this table are priority list (PL); dynamic programming (DP); Lagrangian relaxation (LR); mixed-integer linear programming (MILP); genetic algorithms (GA); simulated annealing (SA); particle swarm optimisation (PSO). Also shown are the power system test setup and maximum number of generators that was used in the study.}
\label{literature:tab:duc_setup}
\end{longtable}
\end{scriptsize}

==> 04-chapter1/tables/10_gen_results.tex <==
\begin{tabular}{lrrr}
\toprule
                                                   &  Mean cost (\$M) &  Std. cost &  LOLP (%) \\
\midrule
                   10 gen, milp (perfect), perfect &             8.82 &        NaN &     0.000 \\
10 gen, guided, uniform_cost_search, H=4, t=nan... &             9.37 &       0.84 &     0.128 \\
                      10 gen, milp (4 sigma), None &             9.40 &       1.02 &     0.180 \\
\bottomrule
\end{tabular}


==> 04-chapter1/tables/20_gen_results.tex <==
\begin{tabular}{lrrr}
\toprule
                                                   &  Mean cost (\$M) &  Std. cost &  LOLP (%) \\
\midrule
                   20 gen, milp (perfect), perfect &            17.58 &        NaN &     0.000 \\
20 gen, guided, uniform_cost_search, H=4, t=nan... &            18.73 &       1.41 &     0.107 \\
                      20 gen, milp (4 sigma), None &            18.90 &       2.92 &     0.244 \\
\bottomrule
\end{tabular}


==> 04-chapter1/tables/30_gen_results.tex <==
\begin{tabular}{lrrr}
\toprule
                                                   &  Mean cost (\$M) &  Std. cost &  LOLP (%) \\
\midrule
                   30 gen, milp (perfect), perfect &            26.31 &        NaN &     0.000 \\
30 gen, guided, uniform_cost_search, H=4, t=nan... &            28.41 &       2.04 &     0.142 \\
                      30 gen, milp (4 sigma), None &            28.53 &       4.94 &     0.291 \\
\bottomrule
\end{tabular}


==> 04-chapter1/tables/all_best_results.tex <==
\begin{tabular}{rlrrr}
\toprule
 Num. gens &         Version &  Mean cost (\$M) &  Std. cost &  LOLP (\%) \\
\midrule
        10 &   MILP(perfect) &             8.82 &       0.00 &      0.000 \\
        10 &      Guided UCS &             9.37 &       0.84 &      0.128 \\
        10 & MILP($4\sigma$) &             9.40 &       1.02 &      0.180 \\
        20 &   MILP(perfect) &            17.58 &       0.00 &      0.000 \\
        20 &      Guided UCS &            18.73 &       1.41 &      0.107 \\
        20 & MILP($4\sigma$) &            18.90 &       2.92 &      0.244 \\
        30 &   MILP(perfect) &            26.31 &       0.00 &      0.000 \\
        30 &      Guided UCS &            28.41 &       2.04 &      0.142 \\
        30 & MILP($4\sigma$) &            28.53 &       4.94 &      0.291 \\
\bottomrule
\end{tabular}


==> 04-chapter1/tables/test_problems_20.tex <==
\begin{tabular}{llrrr}
\toprule
      Date & Day &  Wind (\%) &  $D_{\text{min}}$ (MW) &  $D_{\text{max}}$ (MW) \\
\midrule
2016-01-12 & Tue &       11.0 &                 1981.8 &                 3186.1 \\
2016-07-25 & Mon &       21.7 &                 1580.4 &                 2237.0 \\
2016-11-21 & Mon &       18.1 &                 1945.1 &                 3090.6 \\
2017-03-18 & Sat &       21.3 &                 1655.0 &                 2507.8 \\
2017-04-07 & Fri &        7.4 &                 1760.4 &                 2428.4 \\
2017-05-12 & Fri &       14.4 &                 1734.9 &                 2353.7 \\
2017-05-26 & Fri &       14.8 &                 1634.7 &                 2117.3 \\
2017-06-25 & Sun &        2.8 &                 1400.6 &                 1908.2 \\
2017-12-18 & Mon &        8.1 &                 2023.2 &                 3199.9 \\
2017-12-30 & Sat &       18.4 &                 1832.8 &                 2637.4 \\
2018-01-15 & Mon &       15.0 &                 1786.6 &                 3026.5 \\
2018-03-08 & Thu &        7.0 &                 2048.3 &                 3019.6 \\
2018-03-18 & Sun &       36.8 &                 1887.2 &                 2865.2 \\
2018-05-30 & Wed &       16.5 &                 1565.7 &                 2354.2 \\
2018-09-11 & Tue &       30.8 &                 1599.2 &                 2367.6 \\
2018-11-13 & Tue &       31.1 &                 1705.2 &                 2819.6 \\
2019-04-03 & Wed &       15.6 &                 1802.0 &                 2612.6 \\
2019-05-22 & Wed &       10.1 &                 1638.1 &                 2209.6 \\
2019-10-30 & Wed &        9.5 &                 1877.6 &                 2828.3 \\
2019-11-09 & Sat &        8.9 &                 1837.0 &                 2713.4 \\
\bottomrule
\end{tabular}


==> 04-chapter1/tables/test_problems_30.tex <==
\begin{tabular}{llrrr}
\toprule
      Date & Day &  Wind (\%) &  $D_{\text{min}}$ (MW) &  $D_{\text{max}}$ (MW) \\
\midrule
2016-01-12 & Tue &       11.0 &                 2972.7 &                 4779.2 \\
2016-07-25 & Mon &       21.7 &                 2370.5 &                 3355.4 \\
2016-11-21 & Mon &       18.1 &                 2917.6 &                 4636.0 \\
2017-03-18 & Sat &       21.3 &                 2482.5 &                 3761.8 \\
2017-04-07 & Fri &        7.4 &                 2640.6 &                 3642.6 \\
2017-05-12 & Fri &       14.4 &                 2602.4 &                 3530.6 \\
2017-05-26 & Fri &       14.8 &                 2452.1 &                 3176.0 \\
2017-06-25 & Sun &        2.8 &                 2100.9 &                 2862.3 \\
2017-12-18 & Mon &        8.1 &                 3034.7 &                 4799.8 \\
2017-12-30 & Sat &       18.4 &                 2749.2 &                 3956.1 \\
2018-01-15 & Mon &       15.0 &                 2679.9 &                 4539.7 \\
2018-03-08 & Thu &        7.0 &                 3072.4 &                 4529.4 \\
2018-03-18 & Sun &       36.8 &                 2830.8 &                 4297.9 \\
2018-05-30 & Wed &       16.5 &                 2348.6 &                 3531.2 \\
2018-09-11 & Tue &       30.8 &                 2398.7 &                 3551.3 \\
2018-11-13 & Tue &       31.1 &                 2557.8 &                 4229.4 \\
2019-04-03 & Wed &       15.6 &                 2703.1 &                 3918.9 \\
2019-05-22 & Wed &       10.1 &                 2457.1 &                 3314.4 \\
2019-10-30 & Wed &        9.5 &                 2816.4 &                 4242.5 \\
2019-11-09 & Sat &        8.9 &                 2755.5 &                 4070.1 \\
\bottomrule
\end{tabular}


==> 04-chapter1/tables/test_problems_5.tex <==
\begin{tabular}{llrrr}
\toprule
      Date & Day &  Wind (\%) &  $D_{\text{min}}$ (MW) &  $D_{\text{max}}$ (MW) \\
\midrule
2016-01-12 & Tue &       11.0 &                  495.4 &                  796.5 \\
2016-07-25 & Mon &       21.7 &                  395.1 &                  559.2 \\
2016-11-21 & Mon &       18.1 &                  486.3 &                  772.7 \\
2017-03-18 & Sat &       21.3 &                  413.8 &                  627.0 \\
2017-04-07 & Fri &        7.4 &                  440.1 &                  607.1 \\
2017-05-12 & Fri &       14.4 &                  433.7 &                  588.4 \\
2017-05-26 & Fri &       14.8 &                  408.7 &                  529.3 \\
2017-06-25 & Sun &        2.8 &                  350.2 &                  477.1 \\
2017-12-18 & Mon &        8.1 &                  505.8 &                  800.0 \\
2017-12-30 & Sat &       18.4 &                  458.2 &                  659.4 \\
2018-01-15 & Mon &       15.0 &                  446.7 &                  756.6 \\
2018-03-08 & Thu &        7.0 &                  512.1 &                  754.9 \\
2018-03-18 & Sun &       36.8 &                  471.8 &                  716.3 \\
2018-05-30 & Wed &       16.5 &                  391.4 &                  588.5 \\
2018-09-11 & Tue &       30.8 &                  399.8 &                  591.9 \\
2018-11-13 & Tue &       31.1 &                  426.3 &                  704.9 \\
2019-04-03 & Wed &       15.6 &                  450.5 &                  653.1 \\
2019-05-22 & Wed &       10.1 &                  409.5 &                  552.4 \\
2019-10-30 & Wed &        9.5 &                  469.4 &                  707.1 \\
2019-11-09 & Sat &        8.9 &                  459.2 &                  678.4 \\
\bottomrule
\end{tabular}


==> 05-chapter2/tables/ep_times_summary.tex <==
\begin{tabular}{lrrrrr}
\toprule
{} & \multicolumn{5}{l}{Time (s)} \\
{} &     mean & median &   min &    max &   std \\
Gens &          &        &       &        &       \\
\midrule
10   &     51.8 &   29.8 &   5.7 &  195.8 &  52.3 \\
20   &     41.8 &   34.8 &   7.7 &  159.3 &  35.8 \\
30   &     69.4 &   72.6 &  14.5 &  164.4 &  45.1 \\
\bottomrule
\end{tabular}


==> 05-chapter2/tables/heuristic_run_time.tex <==
\begin{tabular}{lr}
\toprule
        Method &  Mean time (ms) \\
\midrule
    Naive MMFC &        0.615604 \\
      Naive ED &        1.801883 \\
Constrained ED &        2.037926 \\
\bottomrule
\end{tabular}


==> 05-chapter2/tables/rolling_horizon_comp.tex <==
\begin{tabular}{lrrr}
\toprule
{} &  Rolling Horizon &  Day Ahead &  Perfect MILP \\
Gens &                  &            &               \\
\midrule
10   &           10.761 &     10.858 &        10.761 \\
20   &           21.553 &     21.732 &        21.526 \\
30   &           32.285 &     32.553 &        32.304 \\
\bottomrule
\end{tabular}


==> 06-chapter3/tables/carbon_milp_runtime.tex <==
\begin{tabular}{lrrrr}
\toprule
Num. gens &  \$/tCO$_2$ &  Mean time(s) &  Min. time &  Max. time \\
\midrule
       10 &           0 &         19.10 &       1.75 &     177.21 \\
       10 &          50 &         85.70 &       1.78 &     420.50 \\
       20 &           0 &          5.47 &       3.83 &       8.39 \\
       20 &          50 &         38.99 &       3.58 &     458.73 \\
       30 &           0 &          8.03 &       5.58 &      12.42 \\
       30 &          50 &         12.36 &       5.63 &      37.03 \\
\bottomrule
\end{tabular}


==> 06-chapter3/tables/curtailment_results.tex <==
\begin{tabular}{rrrrrrrrr}
\toprule
 $CP$ [\$/tCO$_2$] &  Cost (\$M) &  LOLP (\%) &  ktCO$_2$ &  Curtailment (\%) &  Startups &  Coal &  Gas &  Oil \\
\midrule
                 0 &       30.89 &       0.10 &   1638.27 &              2.01 &       426 &  2617 & 1273 &  276 \\
                25 &       66.39 &       0.09 &   1282.70 &              1.21 &       280 &  2329 & 1604 &  372 \\
                50 &       98.80 &       0.22 &   1253.66 &              1.30 &       121 &  2284 & 1726 &  451 \\
\bottomrule
\end{tabular}


==> bin/literature_RL.tex <==
\section{Monte Carlo Tree Search}

\subsection{Progressive widening techniques} 

In stochastic domains or large/continuous action space domains, MCTS is difficult to apply due to the size of the search tree. In cases with large or continuous action spaces, it may be impractical to sample all actions at each decision node. In progressive widening \cite{coulom2007computing} (or progressive unpruning \cite{chaslot2008progressive}) actions are gradually added to the decision node as the search progresses. The number of actions increases with the number of visits to the decision node, gradually increasing the breadth of the subtree. Actions may be enumerated using prior knowledge of the problem \cite{coulom2007computing, teytaud2009creating} or chosen randomly \cite{wang2009algorithms}. This approach has been used for several games. 

In the case of stochastic transitions, that is where there is a one-to-many mapping of $(s_t, a_t) \rightarrow s_{t+1}$, it is necessary to consider an extra layer of nodes (often called random or chance nodes) corresponding to the possible realisations of the $(s,a)$ pair. Similarly it is often impractical or impossible (as in continuous state spaces) to visit all of the state realisations. Selecting a subset of the state realisations is used to solve Klondike \cite{bjarnason2009lower} which limits the number of states to a fixed width $w$. The width $w$ determines the branching of the search tree and is shown to have a significant impact on the efficacy of MCTS \cite{bjarnason2009lower}. 

The two ideas of using progressive widening for both state and action spaces are combined in polynomial UCT, which double progressive widening (DPW) to gradually increase the search width $w$ at both decision nodes and random nodes \cite{couetoux2011continuous}. Applied to an energy stock management in \cite{couetoux2011adding}, MCTS without DPW is shown to fail in continuous state space: it simply builds a tree of search depth $1$, corresponding to different realisations of each $(s,a)$. MCTS-DPW is effective in solving the energy stock management with random forced outages of thermal generation \cite{couetoux2011adding}.

While it is common to apply heuristic knowledge to enumerating the action space, only limited research has considered how states can be selected intelligently. One approach not discussed in this thesis is to draw from the literature of scenario reduction tools, reducing a large populations of states to a smaller number that approximate the statistical characteristics of the population. 

\section{Microgrids}

Applications of RL to the problem of microgrid management in \cite{franccois2016deep, ji2019real, kuznetsova2013reinforcement} bear more similarities to more modern breakthroughs in RL research, such as \cite{mnih2013playing, silver2018general}.  In this problem domain, a system operator typically controls a combination of generation and storage assets and is connected bi-directionally to the large transmission network, allowing it to buy or sell power based on a price forecast. The task is to operate the microgrid at lowest cost. All of the above approaches succeed in decreasing operating costs with respect to baselines.

Microgrid management is in some respects similar to the UC problem, requiring consideration of forecasts to determine optimal behaviours. In the UC problem, the action space is typically larger due to a greater number of assets and the resulting combinatorial action space. Also, the microgrid domain does not require balancing of supply and demand.

The research in this area has demonstrated that RL is a viable methodology on small power systems, but there has been limited research into the scalability of these approaches to larger problems. In addition, many modern RL techniques have not been applied at all and to the best of our knowledge there have not been attempts to apply self-play deep RL to the stochastic UC problem.

 

